A polarization study of jets interacting with turbulent magnetic fields

We investigate the effect of the jet's immediate surroundings on the non-thermal synchrotron emission and its polarization properties. The ambient medium is equipped with a turbulent magnetic field, which is compressed and amplified by the jets as they progress. This leads to high polarization at the forward shock surface. The randomness in the magnetic polarities of the external fields in the shocked ambient medium (SAM) results in vector cancellation of the polarized components from the jet, thereby causing depolarization of the radiation from the cocoon. We find that due to the slow decay of the fields in the SAM, such depolarization by the fields with large correlation lengths is more prominent when compared to the small-scale fields. Also, the low-power jets, which have magnetic fields comparable in strength to those in the SAM, are more severely affected by the SAM's depolarizing effect, than the high-power ones. The turbulent backflows in the cocoon, as well as the shearing of fields near the contact discontinuity, strengthen the poloidal component in the jet. This causes internal depolarization due to the cancellation of the orthogonally polarized components along the Line of Sight as the field transitions from ordered toroidal to poloidal. The synchrotron maps display high-emission filaments in the cocoon with magnetic fields aligned along them. The kink instability leads to the wiggling motion of the jet's spine, resulting in hotspot complexes in low-power sources.

==> extra_plot.tex <==
\begin{figure*}
\centerline{
\def\arraystretch{1.0}
\setlength{\tabcolsep}{0.0pt}
\begin{tabular}{lcr}
    \includegraphics[width=0.75\linewidth]{PF_43_90deg.pdf}
     \end{tabular}}   
     
     \centerline{
\def\arraystretch{1.0}
\setlength{\tabcolsep}{0.0pt}
\begin{tabular}{lcr}
    \includegraphics[width=0.75\linewidth]{PF_44_90deg.pdf}
     \end{tabular}}   
     
 \centerline{
\def\arraystretch{1.0}
\setlength{\tabcolsep}{0.0pt}
\begin{tabular}{lcr}
    \includegraphics[width=0.75\linewidth]{PF_45_90deg.pdf}
     \end{tabular}}    
     \caption{\REF{1D mean polarization fractions ($\pi_T$ and $\pi_J$) by taking mean along the $Z$-direction as a function of $Y$ at $\theta_I=90^\circ$ image plane. The times for the different snapshots are similar to the Fig.~\ref{fig:inc_42}, ~\ref{fig:diff_len_43},~\ref{fig:diff_len_44} and~\ref{fig:diff_len_45}.}}
     \label{fig:PF_plots}
\end{figure*}

